MOCZ for Blind Short-Packet Communication: Some Practical Aspects

We will investigate practical aspects for a recently introduced blind (noncoherent) communication scheme, called modulation on conjugate-reciprocal zeros (MOCZ), which enables reliable transmission of sporadic and short-packets at ultra-low latency in unknown wireless multipath channels, which are static over the receive duration of one packet. Here the information is modulated on the zeros of the transmitted discrete-time baseband signal's $z-$transform. Due to ubiquitous impairments between transmitter and receiver clocks a carrier frequency offset (CFO) will occur after a down-conversion to the baseband, which results in a common rotation of the zeros. To identify fractional rotations of the base angle in the zero-pattern, we propose an oversampled direct zero testing decoder to identify the most likely one. Integer rotations correspond to cyclic shifts of the binary message, which we compensate by a cyclically permutable code (CPC). Additionally, the embedding of CPCs into cyclic codes, allows to exploit additive error correction which reduces the bit-error-rate tremendously. Furthermore, we use the trident structure in the signals autocorrelation to estimate timing offsets and the channels effective delay spread. We finally demonstrate how these impairment estimations can be largely improved by receive antenna diversity, which enables extreme bursty reliable communication at low latency and SNR.

==> SIMO.tex <==
\section{Multiple Receive Antennas}

If the receiver has $M$ antennas, we can exploit receive antenna diversity, since each antenna will receive the
MOCZ symbol over an independent channel realization.  

We assume
%
\begin{itemize}
  \item All received signals arrive at the same time at the $M$ antennas. Hence all have the same timing offset.  (dense
    Antenna Array, fixed relative antenna positions (no movements))
  \item Each antenna observes an independent channel realization $\vh_m$
  \item The maximal channel delay $L$ is equal for all $M$ antennas.
\end{itemize}
Since the transmission throughout the multipath channel is in the passband $[f_c-\frac{1}{W},f_c+\frac{1}{W}]$, we have
to down convert at the receiver to the baseband $[-\frac{1}{W},\frac{1}{W}]$. Using one clock for all $M$ received
passband signals $y^{(p)}_m(t)$ for $m=1,\dots,M$ will lead to the same CFO for all discrete-time signals
%
\begin{align}
  \hy_{m,k}= e^{\im 2\pi \phi n} y_{m,k}
\end{align}
%
resulting in $M$ rotated zero-codewords $e^{\im\phi}\valp_m$.  As in \secref{sec:fractionalCFO} we can estimate the
common fractional carrier frequency offset by \eqref{eq:fractionalCFOestimater}
%
\begin{align}
  \hat{q}= \arg\min_{q\in[Q]} \sum_{k=1}^K \min\left\{\sum_{m=1}^M|\Fmatrix_{QK} \vtD_R \vy_m|_{Qk\oplus_{\tN} q},
  \sum_{m=1}^M |\Fmatrix_{QK} \vtD_R \cc{\vy^-}_m|_{Qk\oplus_{\tN} q}\right\}\label{eq:fractionalCFOestimaterSIMO}.
\end{align}




%
%\begin{figure}[H]
%  \vspace{-3ex}
%  \begin{subfigure}[b]{0.47\textwidth}
%  \includegraphics[width=0.9\textwidth]{_HuffmanBMOCZ-BCH-31-16andDiZeTK_32BLERoverrSNRindBrunpp70000.eps} 
% %
%\end{subfigure}
%\begin{subfigure}[b]{0.46\textwidth}
%\includegraphics[width=0.9\textwidth]{_HuffmanBMOCZ-BCH-31-16andDiZeTK_32BERoverrSNRindBrunpp70000.eps}\end{subfigure}
%\begin{subfigure}[c]{\textwidth}
%  \centering
%\includegraphics[width=.6\textwidth]{_HuffmanBMOCZ-BCH-31-16andDiZeTK_32BERoverEbN0indBrunpp70000.eps}\end{subfigure}
%\vspace{-2ex}
%\caption{SIMO for $M=1,2,4$ receive antennas over $70$k runs per SNR at $p=1$}\label{fig:simober}
%\vspace{-7ex}
%\end{figure}
%%
%\begin{figure}[H]
%  \begin{subfigure}[b]{0.47\textwidth}
%  %\hspace{-2ex}
%  \includegraphics[width=0.95\textwidth]{BMOCZ_CFO_TO_ACPC_K31B16_BLERrSNR_100k.eps}\end{subfigure}
%\begin{subfigure}[b]{0.47\textwidth}
%\includegraphics[width=0.95\textwidth]{BMOCZ_CFO_TO_ACPC_K31B16_BERrSNR_100k.eps} \end{subfigure}
%\begin{subfigure}[c]{\textwidth}
%  \centering
%\includegraphics[width=.67\textwidth]{BMOCZ_CFO_TO_ACPC_K31B16_BEREbN0_100k.eps}\end{subfigure}
%\vspace{-2ex}
%\caption{SIMO for $M=1,2,4,8,16$, random CFO and STO over $100$k runs%per $\SNR$ at $\pd\!=\!1$
%.}\label{fig:CFO_TO_simo}
%\vspace{-4ex}
%\end{figure}



